Quadrature-Induced Local Minima in Structure-Preserving Lotka-Volterra Control

We study how the choice of harvest quadrature affects optimal control in a positivity-preserving Lotka--Volterra scheme. With harvesting alone, counting the prey removed at each step gives a strictly convex cost. Using the prey density at the start of the step overestimates the catch and can create a strict local minimum with cost above the global minimum. We certify the global minimizers in a two-step example by rational root isolation. A second example shows that, with both species present and positive diffusion, a strict local minimizer for the old-state rule admits a descent direction under the flux rule. For nonnegative $H^1$ initial data and positive diffusivities in one space dimension, the two rules give costs, weighted gradients and Hessians that differ by $O(\tau)$ at the same control, uniformly in the spatial mesh. Here $\tau$ is the time step. If the old-state Hessian is uniformly coercive near a stationary control, the flux objective has a local minimizer within $O(\tau)$ of it. With uniformly bounded tracking targets, a large enough effort penalty makes both objectives strongly convex for all sufficiently small time steps. We also derive exact discrete adjoints and Hessian actions, prove a common variational limit with an IMEX discretization, and compare stationary controls across grids. The same harvest accounting applies to weighted production--destruction systems.

==> tables/algorithms.tex <==
\begin{tabular}{llrrrrrl}
\toprule
Problem & Method & Objective & Iter. & State & Adjoint & $\|R\|_\infty$ & Accepted \\
\midrule
I & L-BFGS-B & -1.549058144 & 83 & 103 & 103 & $9.95\times10^{-8}$ & yes \\
I & FBS & -1.549058144 & 1191 & 1192 & 1192 & $9.96\times10^{-7}$ & yes \\
I & Anderson-FBS & -1.549058144 & 312 & 313 & 313 & $9.94\times10^{-7}$ & yes \\
I & SPG & -1.549058144 & 226 & 228 & 227 & $9.86\times10^{-7}$ & yes \\
$P_0$ & L-BFGS-B & -1.594913505 & 1427 & 1468 & 1468 & $6.25\times10^{-7}$ & yes \\
$P_0$ & FBS & -1.594433433 & 12000 & 12001 & 12001 & $1.03\times10^{-2}$ & no \\
$P_0$ & Anderson-FBS & -1.572467859 & 12000 & 12001 & 12001 & $5.47\times10^{-2}$ & no \\
$P_0$ & SPG & -1.594681506 & 4198 & 4203 & 4199 & $9.70\times10^{-7}$ & yes \\
$P_1$ & L-BFGS-B & -1.520973681 & 82 & 101 & 101 & $1.32\times10^{-7}$ & yes \\
$P_1$ & FBS & -1.520973681 & 1150 & 1151 & 1151 & $9.96\times10^{-7}$ & yes \\
$P_1$ & Anderson-FBS & -1.520973681 & 415 & 416 & 416 & $9.95\times10^{-7}$ & yes \\
$P_1$ & SPG & -1.520973681 & 394 & 396 & 395 & $9.88\times10^{-7}$ & yes \\
\bottomrule
\end{tabular}


==> tables/coarse.tex <==
\begin{tabular}{rlrrrr}
\toprule
$N$ & Problem & $\min v_i$ & Own-grid objective & Common validation & $\|R\|_\infty$ \\
\midrule
4 & I & -0.403868 & -1.653732 & 0.447751 & $6.41\times10^{-8}$ \\
4 & $P_0$ & 0.026532 & -1.851500 & 1.255105 & $1.28\times10^{-9}$ \\
4 & $P_1$ & 0.027097 & -0.757644 & -0.256248 & $2.86\times10^{-8}$ \\
8 & I & 0.010214 & -1.523392 & -0.781285 & $5.57\times10^{-8}$ \\
8 & $P_0$ & 0.027226 & -2.049194 & 0.154229 & $5.85\times10^{-10}$ \\
8 & $P_1$ & 0.029031 & -1.113052 & -0.716974 & $4.67\times10^{-8}$ \\
20 & I & 0.019105 & -1.525015 & -1.439715 & $1.07\times10^{-7}$ \\
20 & $P_0$ & 0.025411 & -1.824709 & -1.157508 & $1.45\times10^{-16}$ \\
20 & $P_1$ & 0.025432 & -1.362237 & -1.346879 & $1.02\times10^{-7}$ \\
\bottomrule
\end{tabular}


==> tables/derivatives.tex <==
\begin{tabular}{lrrrr}
\toprule
Problem & $E_1$ order & $E_g$ order & $E_2$ order & Symmetry defect \\
\midrule
I & 2.008 & 2.001 & 3.003 & $8.67\times10^{-19}$ \\
$P_0$ & 2.010 & 2.003 & 3.004 & $8.67\times10^{-19}$ \\
$P_1$ & 2.009 & 2.002 & 3.004 & $4.34\times10^{-19}$ \\
\bottomrule
\end{tabular}


==> tables/fixed.tex <==
\begin{tabular}{lrrrrr}
\toprule
Study & $N$ or $M$ & IMEX difference & Order & Positive difference & Order \\
\midrule
time & 60 & $5.745\times10^{-2}$ & 1.090 & $1.469\times10^{-1}$ & 0.993 \\
 & 120 & $2.698\times10^{-2}$ & 1.043 & $7.378\times10^{-2}$ & 1.007 \\
 & 240 & $1.310\times10^{-2}$ & 1.021 & $3.671\times10^{-2}$ & 1.006 \\
 & 480 & $6.455\times10^{-3}$ & -- & $1.829\times10^{-2}$ & -- \\
space & 20 & $1.165\times10^{-2}$ & 2.023 & $1.162\times10^{-2}$ & 2.022 \\
 & 40 & $2.866\times10^{-3}$ & 2.006 & $2.860\times10^{-3}$ & 2.006 \\
 & 80 & $7.135\times10^{-4}$ & 2.002 & $7.121\times10^{-4}$ & 2.002 \\
 & 160 & $1.782\times10^{-4}$ & -- & $1.778\times10^{-4}$ & -- \\
\bottomrule
\end{tabular}


==> tables/grids.tex <==
\begin{tabular}{rrrrrrr}
\toprule
$N$ & $j^{\rm I}$ & $j^{P_0}$ & $j^{P_1}$ & $D_0$ & $D_1$ & $\|R^{P_0}\|_\infty$ \\
\midrule
30 & -1.53245751 & -1.74334796 & -1.42279895 & 1.02502 & 0.25743 & $0$ \\
60 & -1.54272250 & -1.65105635 & -1.48709517 & 1.03773 & 0.13552 & $1.30\times10^{-8}$ \\
120 & -1.54905814 & -1.59491350 & -1.52097368 & 1.03898 & 0.07003 & $6.25\times10^{-7}$ \\
240 & -1.55249731 & -1.56621407 & -1.53838209 & 0.51733 & 0.03564 & $1.33\times10^{-7}$ \\
480 & -1.55428314 & -1.56057729 & -1.54720669 & 0.09960 & 0.01796 & $1.17\times10^{-7}$ \\
960 & -1.55519216 & -1.55827777 & -1.55164916 & 0.04775 & 0.00901 & $2.04\times10^{-7}$ \\
\bottomrule
\end{tabular}


==> tables/multistart.tex <==
\begin{tabular}{lrrrr}
\toprule
Problem & Accepted starts & Objective spread & Max. distance to zero start & Largest residual \\
\midrule
I & 5/5 & $2.66\times10^{-15}$ & $3.08\times10^{-7}$ & $4.26\times10^{-7}$ \\
$P_0$ & 5/5 & $8.02\times10^{-4}$ & $1.42\times10^{0}$ & $9.82\times10^{-7}$ \\
$P_1$ & 5/5 & $1.78\times10^{-15}$ & $2.00\times10^{-7}$ & $3.19\times10^{-7}$ \\
\bottomrule
\end{tabular}


==> tables/reference.tex <==
\begin{tabular}{lrrrrrr}
\toprule
Problem & Own-grid objective & Common validation & $\|R\|_\infty$ & $|F|$ & ${\rm TV}_t$ & $\min v_i$ \\
\midrule
I & -1.549058144 & -1.553167396 & $9.95\times10^{-8}$ & 3127 & 2.252 & 0.02198 \\
$P_0$ & -1.594913505 & -1.516824057 & $6.25\times10^{-7}$ & 18 & 19.111 & 0.02306 \\
$P_1$ & -1.520973681 & -1.549474465 & $1.32\times10^{-7}$ & 3076 & 2.232 & 0.02305 \\
\bottomrule
\end{tabular}


==> tables/spectra.tex <==
\begin{tabular}{lrrrrrr}
\toprule
Problem & $\widehat\mu_{\min}$ & $\widehat\mu_{\max}$ & $\widehat\theta_{\max}$ & $\widehat\theta_{\rm opt}$ & $\widehat\rho_{\rm opt}$ & Smallest-mode residual \\
\midrule
I & 0.0473722 & 10.4163839 & 0.0096003 & 0.0095568 & 0.990945 & $4.27\times10^{-8}$ \\
$P_0$ & 0.0027523 & 0.0855827 & 1.1684608 & 1.0000000 & 0.944954 & $1.70\times10^{-17}$ \\
$P_1$ & 0.0501649 & 9.5878358 & 0.0104299 & 0.0103756 & 0.989590 & $4.92\times10^{-8}$ \\
\bottomrule
\end{tabular}

